An alternative approach to Shnirelman's inequality

In this paper we examine the discrete Shnirelman's inequality [Shnirelman A., 1985], which relates the $L^2$-distance of two discrete configurations of a fluid to the $L^1_tL^2_x$-norm of the vector field connecting them. Our proof is inspired by [Shnirelman A., 1985], where it was obtained $\alpha=\frac{1}{64}$ in dimension $\nu=2$, while here we get $\alpha\geq\frac{2}{7}$. Moreover we prove that $\alpha\geq\frac{1}{\nu+1}$ for any dimension $\nu\geq 3$. We point out that, even if this does not improve the bound in the continuous version, where it was proved that $\alpha\geq\frac{2}{4+\nu}$, with $\nu\geq 3$, our bound is the best one achieved for the $2$-dimensional case. Our method uses an alternative approach based on volume estimates of permutations, which count the number of maximum cubes that are moved by a permutation $P$.

==> connettibilita.tex <==
\begin{proposition}\label{prop:male:malissimo}
    Consider the unit cube $[0,1]^2$, the tiling $\mathcal{R}_a$ for some $a>0$ and two colorings $\Pi,\Pi':[0,1]^2\rightarrow\lbrace 0,1\rbrace$ w.r.t. the tiling $\mathcal{R}_a$ into black and white cubes such that
    \begin{equation*}
        \sharp\lbrace\kappa:\Pi(\kappa)=1\rbrace=\sharp\lbrace\kappa:\Pi'(\kappa)=1\rbrace\leq \frac{1}{a}.
    \end{equation*}
    Then there exists a discrete flow $\lbrace Z_j\rbrace$ such that it connects $\Pi,\Pi'$ with the property that each white cube $\kappa\in\mathcal{R}_a$ is displaced no more than $a$, and the cost is computed as
    \begin{equation*}
        L(\Pi,\Pi')\lesssim \sqrt{\sharp\lbrace\kappa:\Pi(\kappa)=1\rbrace a^2}\frac{1}{a}.
    \end{equation*}
\end{proposition}
\begin{proof}
    Call $\frac{1}{a}=M$. If we call $\kappa_{ij}$ the cubes of the tiling, with $i$ referring to the horizontal component and $j$ referring to the vertical one ($i,j=1,2,\dots,M$), we can assume without loss of generality that $\Pi'$ is
    \begin{equation*}
        \Pi'(\kappa_{ii})=1\quad\forall i,
    \end{equation*}
    and zero otherwise (that is, the black cubes are those on the diagonal). Moreover, always w.l.o.g. we can assume that, if $\Pi(\kappa_{ii})=0$, then $\Pi(\kappa_{ij})=\Pi(\kappa_{ji})=0$ for all (indeed, if in any horizontal or vertical column there is a black cube, we can move the closest one to the diagonal position). Our aim is to find paths of maximum length $C$, where $C>0$ is a positive constant, that start in a white cube $\kappa_{ii}$ and that end up in a black cube $\kappa_{hk}$ with $\Pi(\kappa_{hk})=1$, such that they do not self-intersect, and every cube in the path is white. We will indicate paths from $\kappa_{ii},\kappa_{hk}$ indicating the coordinates of the cubes along the path, as $\lbrace (i,i),(i+1,i),\dots, (h,k)\rbrace.$ We will now give the construction of paths. We start with $\kappa_{11}$. If $\Pi(\kappa_{11})=0$ then we cancel the two columns $\cup_{j}\kappa_{1j}\cup _{i}\kappa{i1}$, thus we can assume $\Pi(\kappa_{11})=1$. We construct the paths inductively as follows:
    \begin{itemize}
        \item we define 
        \begin{equation*}
            i_1=\min\lbrace i:\Pi(\kappa_{ii})=0\rbrace;
        \end{equation*}
        \item consider those cubes $\kappa_{ij}$ with $i\not=j$ such that $i\leq i_1$, $j\leq i_1$: then two possible situations may occur:
        \begin{enumerate}
            \item if there exists among them a black cube, $\Pi(\kappa_{ij})$, pick the closest to $\kappa_{i_1i_1}$, and connect the two by a shortest path. (da definire);
            \item if not cut out the set $\cup_{i<i_1}\kappa_{i1}\cup_{j<i_1}\kappa{1j}$ and connect the cube to the "more distant cube" (to define). 
            \item iterate the procedure. 
            \item notice that not all the white cubes can be connected at this stage. But we can estimate the maximum amount that cannot be connected. 
        \end{enumerate}
    \end{itemize}
        
    
\end{proof}

 which will be developed
      in different time steps.
      
      Since the flow will be performed simultaneously and independently on each couple $U_j\cup L_j$, we fix some $j$. We will prove the result in dimension $\nu=2,3$ and we will show how to perform the extension to higher dimension.
      \medskip 
      
      \textbf{Analysis of $\nu=2$. } The analysis here is straightforward since we can rely on the same ideas of Proposition \ref{prop:Step1}. We point out that Assumption A means that the amount of cubes for which $|P(\kappa)-\kappa|>\delta^\epsilon$ can be contained in a single cube of the tiling $\mathcal{R}_{\delta^\epsilon}$. Similarly to what done in Subsection \ref{sss:step:1}, we define
      \begin{equation*}
    \Pi' (\kappa)=\begin{cases}
        0\quad\text{ if } | P(\kappa)-\kappa|\leq\delta^\epsilon, \\
        1 \quad\text{ if } | P(\kappa)-\kappa|>\delta^\epsilon, \\ 
    \end{cases}\kappa\subset U_j.
    \end{equation*}
      Then we perform the following discrete flows (here we remain at the level of the heuristic presentation since the steps are the same of the proposition mentioned above):
      \begin{itemize}
          \item in each subcube of the tiling $\mathcal{R}_{\delta^\epsilon}$ we arrange the colored cubes as in Figure \ref{fig:shn11};
          \item we move the colored cubes  starting from the left horizontally. This is performed in $\delta^{-\epsilon}$ steps. Finally the colored cubes reach the last cube of the tiling;
          \item we define the new coloring
          \begin{equation*}
    \Pi''(\kappa)=\begin{cases}
        0\quad\text{ if } | P(\kappa)-\kappa|\leq\delta^\epsilon, \\
        h \quad\text{ if } | P(\kappa)-\kappa|>\delta^\epsilon,\text{ and } P(\kappa)\in K_{jh}, \\
    \end{cases}
    \end{equation*}
    where we have denoted by $K_{jh}\subset \mathcal{R}_{\delta^\epsilon}$ the cubes contained in $U_j$. Then the flow is constructed as in Figure \ref{fig:prop:shnirel:1}.
      \end{itemize}
   
      These steps, whose total cost is $\delta^{\frac{1}{2}-\frac{3\epsilon}{4}}$, guarantee that at each time step the white cubes are moved only by a constant $C(\nu)\delta^\epsilon$.
      
      \medskip
      \textbf{Analysis of the $\nu\geq 3$ case.}
      For simplicity, we fix $U_j=[0,1]^{\nu-1}\times[0,\delta^\epsilon]$, being $U_j$ a translation of this rectangle. We consider the rectangle $R=[1-\delta^\epsilon,1]\times[0,1]^{\nu-2}\times[0,\delta^\epsilon]$, whose volume is $\delta^{2\epsilon}$. Here, Assumption A means that, given the following coloring
       \begin{equation*}
    \Pi' (\kappa)=\begin{cases}
        0\quad\text{ if } | P(\kappa)-\kappa|\leq\delta^\epsilon, \\
        1\quad \text{ if } | P(\kappa)-\kappa|>\delta^\epsilon, \\ 
    \end{cases}\kappa\subset U_j,
    \end{equation*}
     then the volume of colored cube is less or equal than the volume of $R$. Here we fix $\nu=3$ (the case of higher dimension can be repeated by using the ideas of this case). Call $K_{ih}$ the cubes of the tiling $\mathcal{R}_{\delta^\epsilon}$ contained in $U_j$, more precisely
     \begin{equation*}
         K_{ih}=[0,\delta^\epsilon]^3+ i\delta^\epsilon\mathbf{e}_1+h\delta^\epsilon\mathbf{e}_2,\qquad i,h=0,1,2,\dots\delta^{-\epsilon}-1.
     \end{equation*}
     We first need to prove that, if the coloring $\Pi'$ is such that, for every fixed $K_{ih}$,
     \begin{equation*}
         \Pi'(\kappa)=\text{const},\forall \kappa\subset K_{ih},
     \end{equation*}
     then we can construct a flow that moves all the cubes $K_{ih}$ such that $\Pi'(\kappa)=1$ for all $\kappa\subset K_{ih}$ into the last column $\cup_h{K_{(\delta^{-\epsilon}-1,h)}}$, with the constraint that white cubes do not move more than $C\delta^\epsilon$. We apply Proposition $\ref{prop:male:malissimo}$ with $a=\delta^\epsilon$ to the slice $U_j$ seen as a $2$-dimensional surface. Then each white cube is moved no more than $\delta^{\epsilon}$, the length of path is $\leq 3$ and so the cost here is computed as
     \begin{equation*}
         \sim \sqrt{\delta^{1-\frac{3\epsilon}{2}}\delta^{2\epsilon}}\delta^{-\epsilon}=\sim \delta^{\frac{1}{2}-\frac{3\epsilon}{4}}.
     \end{equation*}
     
     
     
     
     At this stage 
     If we are able to prove this result, we construct a flow acting on each slice $[0,1]\times[0,1]\times[jN^{-1},(j+1)N^{-1}]$ for every $j$ as the one we will propose, then this will end the proof.  
     
     Here we construct our discrete flow:
     \begin{itemize}
         \item In each cube of the tiling $\mathcal{R}_{\delta^\epsilon}$ arrange the colored cubes in the following inductive way (see Figure \ref{fig:shn:cor}):
         \begin{enumerate}
             \item In $K_{(\delta^{-\epsilon}-1)h}$ the black cubes are contained in the slice $S(K_{(\delta^{-\epsilon}-1)h})=[1,1-\delta^\epsilon]\times[h\delta^\epsilon,(h+1)\delta^\epsilon]\times[0,k(K_{\delta^{-\epsilon}h})]$;
             \item in $K_{(\delta^{-\epsilon}-2)h}$ the black cubes are contained in 
             
             $S(K_{(\delta^{-\epsilon}-2)h})=[1,1-\delta^\epsilon]\times[h\delta^\epsilon,(h+1)\delta^\epsilon]\times[k(K_{(\delta^{-\epsilon}-1)h},\min\lbrace k(K_{(\delta^{-\epsilon}-2)h})+k(K_{(\delta^{-\epsilon}-1)h},1\rbrace]\bigcup$
             
             $[1,1-\delta^\epsilon]\times[h\delta^\epsilon,(h+1)\delta^\epsilon]\times[0,\max\lbrace ( k(K_{(\delta^{-\epsilon}-2)h})+k(K_{(\delta^{-\epsilon}-1)h}))-1,0\rbrace]$;
             \item $\dots$.
         \end{enumerate}
         This step is performed at the cost of $\delta^{\frac{1}{2}-\frac{3\epsilon}{4}}\delta^\epsilon$;
         \item move all the slices of black cubes in the last cube $K_{(\delta^{-\epsilon}-1)j}$. This is performed in $\delta^{-\epsilon}$ steps, each one at a cost $\sim \delta^{\frac{1}{2}-\frac{3\epsilon}{4}}\delta^{\epsilon}$ (Theorem \ref{thm:cost:nucube}, Corollary \ref{cor:cost:coloring:rectangles}). Call for simplicity $P$ the permutation obtained at the end of this stage.
         \item Observe that if, fixed $j$, there exists $\bar\kappa\subset K_{(\delta^{-\epsilon}-1)h}$ s.t. $\Pi(\bar\kappa)=0$, (here this $\bar\kappa$ is $\bar\kappa=P(\kappa)$ for some $\kappa\in \mathcal{R}_N$) then $\Pi(\kappa)=0$ for all $\kappa\subset K_{ih}$ for all $i$. This is the case of Figure \ref{fig:shncormorte2}.
         \item In each cube of the tiling $\mathcal{R}_{\delta^\epsilon}$ arrange the colored cubes inductively ad in the previous steps, that is:
         \begin{enumerate}
             \item Take $i=\delta^{-\epsilon}-2$ and let $\bar h_1=\min\lbrace h:\exists \kappa\in K_{ih}:\Pi(\kappa)=1\rbrace$. Arrange the cubes in $K_{ih_1}$ such that they are all contained in the slice $[\delta^{-\epsilon}-2,\delta^{-\epsilon}-1]\times [(h_1-1)\delta^{-\epsilon},h_1\delta^{-\epsilon}\times [0, k(K_{ih_1})]$; etc
         \end{enumerate}
         
        


         
     \end{itemize}
\begin{figure}
    \centering
    \includegraphics[scale=0.75]{shncormorte.png}
    \caption{Subdivision of black cubes in the case $\nu=3$. The red arrows indicate the action of the flow. Clearly, the white cube are moved only by $\delta^\epsilon$. This is reminiscent of the time steps in the proof of Proposition \ref{prop:Step1}.}
    \label{fig:shn:cor}
\end{figure}

      \begin{figure}
             \centering
             \includegraphics[scale=0.7]{shncormorte2.png}
             \caption{After moving all the black cubes in the last column, the discrete flows organize the black cubes in the vertical direction. This is computed as the same cost $\delta^{\frac{1}{2}-\frac{3\epsilon}{4}}\delta^\epsilon$ and repeated in $\sim \delta^{-\epsilon}$ steps. This guarantees that the white cubes are displaced no more than $C\delta^\epsilon$.}
             \label{fig:shncormorte2}
         \end{figure}

==> costcoloring.tex <==
\section{Estimating the cost of swapping cubes}
In this section we prove the main result of the present paper, indeed we propose a variant of the $S$-discrete flow (Definition \ref{def:S:flow}) constructed in \cite{Shnirelman} (see also Subsection \ref{SS:Shnirlm:discrete:action}). The advantage is that the new discrete flow that will be defined in the next section (Definition \ref{def:discrete:flow}), allows to write the Length functional \ref{eq:discr:length} in a easier way. Though the definition we will propose later (Definition \ref{eq:cost:elem:movem}) is equivalent to the swapping of adjacent cubes, it allows to improve the estimates in Shnirelman's inequality. 

We start with the following considerations. We consider a array $A$ of cubes of the tiling $\mathcal{R}_N$ and we ask how can we estimate the \emph{cost} required to swap the first and the last cube. As suggested by Shnirelman's discrete length functional, we expect that the cost for performing this swapping is $\sim \sqrt{2 N^{-\nu} (\ell(A)^2N^{-2})}$, where we recall that $\ell(A)$ is the length of the array $A$. That is, the cost of the swapping is the square root of the total volume of the two cubes times their distance squared. We formalize this fact in the following lemma, where we prove that the swap of two \emph{distant} cubes can be realized as the time-1 map of a divergence-free vector field in $L^1_tL^2_x$. 

The main observation here is that the cost for swapping the two cubes depends only on their volume and on their mutual distance, not on the volumes of the intermediate cubes. With reference to Figure \ref{fig:lemmaS} the flow particles of the first and last cube follow the trajectories living in a small frame, leaving the particles of the intermediate cubes in their original position. We remark that, though all the proofs are given in dimension $\nu=2$ to avoid technicalities, the statement will be given for any dimension $\nu$.
\begin{figure}
    \centering
    \includegraphics[scale=0.7]{lemmaS.png}
    \caption{A particle follows the red trajectory to reach the distant cube.}
    \label{fig:lemmaS}
\end{figure}
\begin{lemma}\label{lem:first:exchange}
   Let us consider a array $A\subset\mathcal{R}_N$ of length $\ell(A)=M$ with $M\geq 1$. If we denote $A=[\kappa_1,\dots,\kappa_M]$, then there exists a divergence-free vector field $\mathbf v\in L^1_tL^2_x\cap  L^1([0,1],\BV([0,1]^\nu))${\color{red} ricordati di scrivere la regolarità su sottinsiemi e scrivere che le notazioni sono tutte abbreviate} with the following property: if $X:[0,1]^\nu\rightarrow [0,1]^\nu$ denotes the time-1 map of the vector field $\mathbf v$, then there exists a positive constant $C>0$, independent of $M,N$ such that 
    \begin{enumerate}
        \item $\|\mathbf v\|_{L^1_tL^2_x}\leq C \sqrt{N^{-\nu-2}M^2}$;
        \item  the map $X$ translates $\kappa_1$ into $\kappa_M$ (and viceversa), remaining constant on $A\setminus \kappa_1\cup\kappa_M$ modulo a set of measure zero, namely \begin{equation*}
        X(x)=\begin{cases} (x_1+MN^{-1}-N^{-1},\dots,x_{\nu-1}, x_\nu ), \quad x\in \text{int}(\kappa_1), \\
        (x_1+N^{-1}-MN^{-1},\dots,x_{\nu-1}, x_\nu) \quad x\in \text{int}(\kappa_M),\\
        x \quad \text{otherwise},
             \end{cases} \quad\L^2-\text{a.e. } x.
    \end{equation*}
    \end{enumerate} 
   
\end{lemma}
\begin{proof}
    We give the proof for $\nu=2$, the extension to higher dimension being straightforward.  Fix $\epsilon>0$ to be chosen later in order to impose the incompressibility condition on the vector field $\mathbf v$. Call
    \begin{equation*}
        a=\frac{\epsilon}{\epsilon+N^{-1}},\qquad b=aMN^{-1},\qquad c=N^{-1}-b;
    \end{equation*}
    then define the following four sets:
     $$A_\epsilon=\left\lbrace (x,y)\in\mathbb R^2: 0\leq y\leq \epsilon,\quad \frac{y}{a}\leq x\leq \frac{y-b}{-a}\right\rbrace,$$
    $$B_\epsilon=\left\lbrace (x,y)\in\mathbb R^2: MN^{-1}-N^{-1}-\epsilon\leq x\leq MN^{-1}, \quad -ax+b\leq y\leq ax+N^{-1}-b\right\rbrace,$$
   $$C_\epsilon=\left\lbrace (x,y)\in\mathbb R^2: N^{-1}-\epsilon\leq y\leq N^{-1}, \quad -\frac{y-N^{-1}}{a}\leq x\leq \frac{y-c}{a}\right\rbrace,$$
    $$D_\epsilon=\left\lbrace (x,y)\in\mathbb R^2: 0\leq  x\leq N^{-1}+\epsilon, \quad ax\leq y\leq -ax+N^{-1}\right\rbrace.$$
    In each one of these sets we define a shear vector field: 
    \begin{equation}\label{eq:vect:field}
        {\mathbf v_1}(x,y)=\begin{cases}
            \left(-\frac{2}{a}y+\frac{b}{a},0\right),\quad (x,y)\in \text{int}(A_\epsilon), \\
            \\
\left(0,2ax+N^{-1}-2b\right),\quad (x,y)\in \text{int}(B_\epsilon), \\
             \\
             \left(-2\frac{y}{a}+\frac{N^{-1}}{a}+\frac{c}{a},0\right),\quad (x,y)\in \text{int}(C_\epsilon), \\
             \\
             \left(0, 2ax-N^{-1}\right),\quad (x,y)\in \text{int}(D_\epsilon). 
        \end{cases}
    \end{equation}
    It can be proved that, with the choice of
   \begin{equation*}
       \epsilon=\frac{N^{-1}}{M-1},
   \end{equation*}
   the vector field is incompressible.
   Indeed, take a test function $\varphi\in\mathcal{C}^\infty_c(A)$, with $\text{supp}(\varphi)\subset A_\epsilon\cup B_\epsilon$ (we can limit ourselves to the study of this case by the symmetry of the problem). Then we have
   \begin{align*}
   0&=\int_{A_\epsilon\cup B_\epsilon} \mathbf { v_1}\cdot\nabla \varphi dx\\&=
   \int_{0}^\epsilon\int_{\frac{y}{a}}^{-\frac{y}{a}+\frac{b}{a}}\left(-\frac{2}{a}y+\frac{b}{a}\right)\partial_1\varphi dxdy +\int_{MN^{-1}-N^{-1}-\epsilon}^{MN^{-1}}\int_{-ax+b}^{ax+N^{-1}-b}(2ax+N^{-1}-2b)\partial_2\varphi dydx\\&=\int_{0}^\epsilon\left(-\frac{2}{a}y+\frac{b}{a}\right)\varphi\left(-\frac{y}{a}+\frac{b}{a},y\right) dy -\int_{MN^{-1}-N^{-1}-\epsilon}^{MN^{-1}}(2ax+N^{-1}-2b)\varphi\left(x,-ax+b\right)dx\\&=\int_{MN^{-1}-N^{-1}-\epsilon}^{MN^{-1}}a\left(2x-\frac{b}{a}\right)\varphi\left(x,-ax+b\right) dx -\int_{MN^{-1}-N^{-1}-\epsilon}^{MN^{-1}}(2ax+N^{-1}-2b)\varphi\left(x,-ax+b\right)dx,
   \end{align*}
   in particular, since the previous equality holds for any choice of the function $\varphi$, we have to require that
   \begin{equation*}
       -b-N^{-1}+2b=0 \longrightarrow \epsilon=\frac{N^{-1}}{M-1}.
   \end{equation*}
   In particular, we remark that $\epsilon$ decreases as the distance between the two cubes increases. 

   \textbf{Step 1.} Since we need to construct the flow that swaps the first and the last cube of the array, we consider $F=A_\epsilon\cup B_\epsilon\cup C_\epsilon\cup D_\epsilon\setminus F'$, where $F'$ is the blue set of Figure \ref{fig:lemmaS2}.
   \begin{figure}
       \centering
       \includegraphics[scale=0.5]{lemmaS2.png}
       \caption{The flow is performed inside the set $A_\epsilon\cup B_\epsilon\cup C_\epsilon\cup D_\epsilon \setminus F',$ where $F'$ denotes the blue frame.}
       \label{fig:lemmaS2}
   \end{figure}
    We consider the flow associated to the vector field defined above, restricted to the set $F$, that is the solution to the Cauchy Problem
    \begin{equation*}
        \begin{cases}
            \dot X(t,(x,y))= \mathbf{ v_1}(X(t, (x,y))), \\
            X(0,(x,y))=(x,y),
        \end{cases}
        (x,y)\in F.
    \end{equation*}
   We observe that in the time interval $t\in[0,2]$ the flow map $X_{t=2}$ has rotated counterclockwise the set $F$ of an angle $\pi$, leaving the intermediate region $A\setminus F$ fixed (see Figure \ref{fig:lemmaS3}). We estimate the $L^2$-norm of the vector field as follows
   \begin{equation*}
       \|\mathbf {v_1}\|^2_{L^2_x}\leq \|\mathbf v_1\|_\infty^2|F|\leq (4M^{2}N^{-2})4N^{-2},
   \end{equation*}
   where we have used that $|F|=2|\kappa_1|+2\frac{N^{-1}}{M} ((M-2)N^{-1}).$
   \begin{figure}
       \centering
       \includegraphics[scale=0.5]{lemmaS3.png}
       \caption{In the time interval $t\in[0,2]$ the flow has rotated counterclockwise the set $F$ of an angle $\pi$. In order to recover the original permutation we have to counter-rotate the set $F$.}
       \label{fig:lemmaS3}
   \end{figure}
   
   \textbf{Step 2.} Here we define the counter rotation vector field. We call
   $$A'_\epsilon=A_\epsilon\setminus (F'\cup (\kappa_1\cup\kappa_M))=[N^{-1},MN^{-1}-N^{-1}]\times\left[0,\frac{N^{-1}}{M}\right],$$
   $$C'_\epsilon=C_\epsilon\setminus (F'\cup (\kappa_1\cup\kappa_M))=[N^{-1},MN^{-1}-N^{-1}]\times\left[N^{-1}-\frac{N^{-1}}{M},N^{-1}\right].$$
    We consider the vector field
   \begin{equation*}
       \mathbf{ v_2}= \mathbf{ v}_{\kappa_1}+\mathbf{ v}_{\kappa_M}+\mathbf{v}_{A'_\epsilon}+\mathbf{v}_{C'_\epsilon},
   \end{equation*}
   where we have used the rotation vector field (Equation \eqref{eq:rot:vf:rectangle}) in the interior of each one of the four sets $\kappa_1,\kappa_M,A'_\epsilon,C'_\epsilon.$ 
 This vector field rotates, in a interval of time $\Delta t=2$, the four sets counterclockwise of an angle $\pi$, as illustrated in Figure {\color{red} fai la figura}. If we estimate the $L^2$-norm of this vector field we find that
 \begin{equation*}
     \|\mathbf{v_2}\|^2_{L^2_x}\leq 2\|\mathbf v_{\kappa_1}\|^2_\infty N^{-2}+2\|\mathbf v_{A'_\epsilon}\|_\infty^2|A'_\epsilon|\leq 4M^2N^{-4}.
 \end{equation*}
 We collect Step 1 and Step 2 defining the vector field of the statement, that is

 \begin{equation*}
     \mathbf v(t,x,y)=\begin{cases}
         8 \mathbf{v_1}(x,y),\quad t\in\left[0,\frac{1}{4}\right), \\
         8 \mathbf{v_2}(x,y), \quad t\in\left[\frac{1}{4},\frac{1}{2}\right).
     \end{cases}
 \end{equation*}
 We could stop the procedure here, since the flow map $T=X_{t=\frac{1}{2}}$ associated to vector field $\mathbf v$ has the following properties:
 \begin{itemize}
     \item $T(\kappa_1)=\kappa_M$ and $T(\kappa_M)=\kappa_1$ and $T\llcorner_{ \kappa_i}$ with $i=1,M$ is a translation;
     \item $T(\kappa_j)=\kappa_j$ for $j\not=1,M$.
 \end{itemize}
So that the map $T$ is a permutation of the cubes of the array. We point out that $T\llcorner_{\kappa_j}$ with $j\not=1,M$ is not the identity. In steps $3$ and $4$ we show how to overcome this issue (that, anyway, is not a issue). 
     \textbf{Step 3.} In this step and the following we correct the map $T$ of the previous two steps such that
     \begin{equation*}
         T\llcorner_{\kappa_j}=Id,\quad \text{a.e. }x,  \quad j\not=1,M. 
     \end{equation*}
     Accordingly to the reference Figure, we define
     \begin{equation*}
         \mathbf{v_3}=\sum_{j=2}^{M-1}  \mathbf v_{\kappa_j}.
     \end{equation*}
     Here the estimate of the $L^2$-norm reads as follows:
     \begin{equation*}
         \|\mathbf{v_3}\|^2_{L^2_x}\leq (M-2)\|v_{\kappa_j}\|^2_\infty |\kappa_j|\leq M^2N^{-4}.
     \end{equation*}
     \textbf{Step 4.}
     For this last step we define
     \begin{equation*}
         \kappa_j^A=\kappa_j\cap A'_{\epsilon},\qquad \kappa_j^C=\kappa_j\cap C'_\epsilon,
     \end{equation*}
     and finally
     \begin{equation*}
         \mathbf{v_4}=\sum_{j=2}^{M-1}\left(\mathbf{v}_{\kappa_j^A}+\mathbf{v}_{\kappa_j^C}+\mathbf{v}_{\kappa_j\setminus(\kappa_j^A\cup\kappa_j^c)}\right).
     \end{equation*}
     Here, the computation of the $L^2$-norm is the same as in Step 3. 

        Finally the vector field of the statement is defined as 
         \begin{equation*}
     \mathbf v(t,x,y)=\begin{cases}
         8 \mathbf{v_1}(x,y), \quad t\in\left[0,\frac{1}{4}\right), \\
         8 \mathbf{v_2}(x,y), \quad 
  t\in\left[\frac{1}{4},\frac{1}{2}\right), \\
         8 \mathbf{v_3}(x,y), \quad t\in\left[\frac{1}{2},\frac{3}{4}\right), \\
         8 \mathbf{v_4}(x,y), \quad t\in\left[\frac{3}{4},1\right).\\
     \end{cases}
 \end{equation*}
        This vector field is clearly $\BV$, divergence-free and satisfies the assumptions of the statement. Moreover, we have that
        \begin{align*}
             \|\mathbf v\|_{L^1_tL^2_x}\leq 2\sum_{h=1}^4\|\mathbf{v_h}\|_{L^2_x},
        \end{align*}
        which, together with the estimates obtained for $\|\mathbf{v_h}\|_{L^2_x}$, gives the statement with constant $C=20$, that clearly depends only on the dimension $\nu=2$. {\color{red} un commento sulla regolarità $\BV$.}
\end{proof}
\begin{remark}
    The parameter $\epsilon$ chosen in the previous proposition can be shown to be 
    \begin{equation*}
        \epsilon\sim \frac{N^{-1}}{M},
    \end{equation*}
    in any dimension $\nu$.
\end{remark}

\begin{remark}
    We point out that, if we consider the permutation $P$ defined as follows:
    \begin{equation*}
        P(\kappa_1)=\kappa_M,\qquad P(\kappa_M)=\kappa_1,
    \end{equation*}
    \begin{equation*}
        P(\kappa_j)=\kappa_j,\quad j\not= 1,M,
    \end{equation*}
    where we are considering the array $A$ in the statement of the previous lemma, then $\|P-Id\|_{L^2}=\sqrt{2|\kappa_1|(MN^{-1})^2}\sim \|\mathbf{v}\|_{L^1_tL^2_x}$. This result tells us that also in the case the permutation swaps distant cubes the cost, computed in terms of the kinetic energy $\|\mathbf v\|_{L^1_tL^2_x}$, is equivalent to the $L^2$-distance of the permutation $P$ from the Identity. 
\end{remark}
\begin{remark}
    We would also remark that the flow map constructed in the previous lemma is non-smooth in the interior of the cubes of the tiling $\mathcal R_N$, differently from what done in \cite{Shnirelman}. Here, indeed, we lose this property, but we gain the advantage that the mass of cubes flows along tubes of size $\epsilon\sim \frac{N^{-1}}{M},$ basically leaving unchanged the mass of the intermediate cubes. Again, this description is equivalent to the one in \cite{Shnirelman}, but, according to us, it gives a more clear picture about the flow of swapping cubes (see also the previous remark). 
 
\end{remark}
The ideas of the previous lemma can be generalized as follows for colorings of arrays in white and black cubes, that is:

\begin{proposition}\label{thm:main:array}
Let $A$ be a array of the tiling $\mathcal{R}_N$ of length $M=\ell(A)$,  and let $\Pi,\tilde\Pi: A\rightarrow\lbrace 0,1\rbrace$ be two colorings of $A$ w.r.t. the tiling $\mathcal{R}_N$ (Definition \ref{def:coloring}) into white and black cubes, with the assumption that they have the same number of black cubes, that is $b=\sharp\lbrace \kappa\in R: \tilde\Pi(\kappa)=1\rbrace=\sharp\lbrace \kappa\in R: \Pi(\kappa)=1\rbrace$. 

Then there exists a divergence-free vector field $\mathbf v\in L^1_t\BV_x\cap L^1_t L^2_x$, $\mathbf v:[0,1]\times [0,1]^\nu\rightarrow\R^\nu$, with the following properties: 
\begin{itemize}
\item if $X$ is the time-1 map of the flow of $\mathbf v$, then $X$ is a permutation of the cubes $\kappa\subset R$ {\color{red} metti definizione di permutazione di $R$};
\item the map $X$ sends the coloring $\Pi$ into $\tilde\Pi$, that is $\tilde\Pi(\kappa)=\Pi( X(\Pi,\tilde\Pi)^{-1}(\kappa))$ for every $\kappa\subset R$;
\item there exists a positive constant $C>0$ depending only on the dimension $\nu$ such that \begin{equation}\label{eq:cost:coloring}\|\mathbf v\|_{L^1_tL^2_x}\leq C \sqrt{2\min(M-b,b)N^{-\nu}}(MN^{-1}).\end{equation}
\end{itemize}
\end{proposition}
\begin{proof}
    {\color{red} serve figura.} Without loss of generality we can assume that $b\leq M-b$ and $\tilde\Pi$ is the canonical coloring \ref{def:canonical:coloring}. 
    We start enumerating the cubes on the array starting from the left as follows: if $\lbrace j\geq 1: \Pi(\kappa_i)=0, \forall i\leq j\rbrace$ we define $\ell_1=0$ and $b_1=\max\lbrace j> \ell_1: \Pi(\kappa_i)=1,\forall <i\leq j, i>\ell_1\rbrace$, if not
    \begin{equation*}
        \ell_1=\max\lbrace j\geq 1: \Pi(\kappa_i)=0, \forall i\leq j\rbrace, \quad b_1=\max\lbrace j> \ell_1: \Pi(\kappa_i)=1,\forall <i\leq j, i>\ell_1\rbrace,
    \end{equation*}
    and inductively
    \begin{equation*}
        \ell_{j+1}=\max\lbrace j\geq b_{j}: \Pi(\kappa_i)=0, \forall i\leq j, i>b_j\rbrace, \quad b_{j+1}=\max\lbrace j> \ell_{j+1}: \Pi(\kappa_i)=1,\forall <i\leq j, i>\ell_{j+1}\rbrace.
    \end{equation*}
    The procedure stops if there exists $1<k\leq M$ such that $\ell_k=0$, $b_{k-1}\not=0$ or $\ell_{k}\not=0$, $b_k=0$. Since the first case is the analogous to the second case with $k-1$ by considering a shorter array of length $M-b_{k}$ (recall that we want to send the coloring $\Pi$ into the canonical coloring), we will assume that
    \begin{equation*}
        \exists k\leq b: \ell_k\not=0, b_k=0.
    \end{equation*}
\end{proof}


==> duration.tex <==
\section{Duration of the longest path}
Hopefully here we prove that the duration of the longest path is $O(N)$. This should give the bound $N^{1+\nu}$. 
